Towards Robust Knowledge Tracing Models via k-Sparse Attention

Knowledge tracing (KT) is the problem of predicting students' future performance based on their historical interaction sequences. With the advanced capability of capturing contextual long-term dependency, attention mechanism becomes one of the essential components in many deep learning based KT (DLKT) models. In spite of the impressive performance achieved by these attentional DLKT models, many of them are often vulnerable to run the risk of overfitting, especially on small-scale educational datasets. Therefore, in this paper, we propose \textsc{sparseKT}, a simple yet effective framework to improve the robustness and generalization of the attention based DLKT approaches. Specifically, we incorporate a k-selection module to only pick items with the highest attention scores. We propose two sparsification heuristics : (1) soft-thresholding sparse attention and (2) top-$K$ sparse attention. We show that our \textsc{sparseKT} is able to help attentional KT models get rid of irrelevant student interactions and have comparable predictive performance when compared to 11 state-of-the-art KT models on three publicly available real-world educational datasets. To encourage reproducible research, we make our data and code publicly available at \url{https://github.com/pykt-team/pykt-toolkit}\footnote{We merged our model to the \textsc{pyKT} benchmark at \url{https://pykt.org/}.}.

==> problem.tex <==
The objective of KT models is given a student's chronologically ordered collection of $T$ past interactions i.e., $\mathbf{S} = \{\mathbf{s}_j\}_{j=1}^T$, 
we aim to predict the probability of whether a student will answer $q_*$ correctly. Specifically, $\mathbf{s}_j$ is a ordering 4-tuple, i.e., $\mathbf{s}_j = <q_j, \mathbf{c}_j, r_j, t_j>$, where $q_j$, $\mathbf{c}_j$, $r_j$ and $t_j$ represent the specific question, the associated KC set, student response \footnote{Response $r_j \in \{0,1\}$, 1 represents the student answered correctly, and 0 otherwise.} and student's response timestamp respectively.


 % arbitrary question $q_*$ to predict the probability of whether a student will answer $q_*$ correctly or not based on the student's historical interaction data. Specifically, for each student $\mathbf{S}$, we assume that we have observed a chronologically ordered collection of $T$ past interactions i.e., $\mathbf{S} = \{\mathbf{s}_j\}_{j=1}^T$. Each interaction is represented as a 4-tuple $\mathbf{s}_j$, i.e., $\mathbf{s}_j = <q_j, \mathbf{c}_j, r_j, t_j>, 0 < t_j < t_{j+1}$, where $q_j$, $\mathbf{c}_j$, $r_j$, $t_j$ represent the specific question, the associated KC set, the binary valued student response\footnote{Response is a binary valued indicator variable where 1 represents the student correctly answered the question, and 0 otherwise.}, and student's response timestamp respectively. We would like to estimate the probability $\hat{r}_{*}$ of the student's performance on arbitrary question $q_*$.
